Dreaming Out Loud: A Self-Synthesis Approach For Training Vision-Language Models With Developmentally Plausible Data

While today's large language models exhibit impressive abilities in generating human-like text, they require massive amounts of data during training. We here take inspiration from human cognitive development to train models in limited data conditions. Specifically we present a self-synthesis approach that iterates through four phases: Phase 1 sets up fundamental language abilities, training the model from scratch on a small corpus. Language is then associated with the visual environment in phase 2, integrating the model with a vision encoder to generate descriptive captions from labeled images. In the "self-synthesis" phase 3, the model generates captions for unlabeled images, that it then uses to further train its language component with a mix of synthetic, and previous real-world text. This phase is meant to expand the model's linguistic repertoire, similar to humans self-annotating new experiences. Finally, phase 4 develops advanced cognitive skills, by training the model on specific tasks such as visual question answering and reasoning. Our approach offers a proof of concept for training a multimodal model using a developmentally plausible amount of data.

==> tables/synthetic_examples.tex <==
% \begin{tabular}{>{\centering\arraybackslash}m{3.2cm} p{4.2cm}}
% \hline
%     image & synthetic description \\
%     \vspace{.5cm}\includegraphics[width=3.2cm]{figures/e1.png} & \vspace{-1cm}Hot off the field at the Ravensboro Golf Club in Ravensboro, IL. I am looking forward to the win of the season. I love the game and hopefully the games are really going to be a big thing...  \\
%     \vspace{.5cm}\includegraphics[width=3.2cm]{figures/e2.png} & \vspace{-1cm}The first section of the East End of London's West End was dedicated to the Holy Spirit. The West End of London's West End was the last part of the East End of London... \\
%     \vspace{.5cm}\includegraphics[width=3.2cm]{figures/e3.png} & \vspace{-1cm}The airport is in the midst of a multi-year, \$10 billion contract with the U.S. Navy, which is expected to be operational over the next few years. The agreement is expected to be signed by the United States, Canada, and the United States... \\
%  \hline
% \end{tabular}

\FloatBarrier
\begin{table*}[htpb!]
\centering
\begin{tabular}{cp{0.7\linewidth}}
\toprule
\textbf{Image} & \textbf{Synthetic Description} \\
\midrule
\includegraphics[width=3cm]{figures/e1.png} & \vspace{-1.7cm} Hot off the field at the Ravensboro Golf Club in Ravensboro, IL. I am looking forward to the win of the season. I love the game and hopefully the games are really going to be a big thing... \\
\includegraphics[width=3cm]{figures/e2.png} & \vspace{-1.7cm} The first section of the East End of London's West End was dedicated to the Holy Spirit. The West End of London's West End was the last part of the East End of London... \\
\includegraphics[width=3cm]{figures/e3.png} & \vspace{-1.7cm} The airport is in the midst of a multi-year, \$10 billion contract with the U.S. Navy, which is expected to be operational over the next few years. The agreement is expected to be signed by the United States, Canada, and the United States... \\
\bottomrule
\end{tabular}
\caption{Synthetic descriptions generated by the model for the images shown. This table illustrates the model's ability to associate visual cues with corresponding textual representations.}
\label{tab:synthetic_desc}
\end{table*}
\FloatBarrier
